Coercivity, hypocoercivity, exponential time decay and simulations for discrete Fokker-Planck equations

In this article, we propose and study several discrete versions of homogeneous and inhomogeneous one-dimensional Fokker-Planck equations. In particular, for these discretizations of velocity and space, we prove the exponential convergence to the equilibrium of the solutions, for time-continuous equations as well as for time-discrete equations. Our method uses new types of discrete Poincar\'e inequalities for a "two-direction" discretization of the derivative in velocity. For the inhomogeneous problem, we adapt hypocoercive methods to the discrete cases.

==> evolfinhom_t-0_cas-L2L2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}
\end{tikzpicture}%
\caption{Initial datum $f^0$ in the inhomogeneous case, the velocity range is $(-20,20)$, the space range is $(0,1)$ the discretization steps are  ${\dvh=0.4}$, ${\dxh=0.01}$ and ${\dth=0.0005}$.}

